Value of Information in Bayesian Routing Games

We study a routing game in an environment with multiple heterogeneous information systems and an uncertain state that affects edge costs of a congested network. Each information system sends a noisy signal about the state to its subscribed traveler population. Travelers make route choices based on their private beliefs about the state and other populations' signals. The question then arises, "How does the presence of asymmetric and incomplete information affect the travelers' equilibrium route choices and costs?'' We develop a systematic approach to characterize the equilibrium structure, and determine the effect of population sizes on the relative value of information (i.e. difference in expected traveler costs) between any two populations. This effect can be evaluated using a population-specific size threshold. One population enjoys a strictly positive value of information in comparison to the other if and only if its size is below the corresponding threshold. We also consider the situation when travelers may choose an information system based on its value, and characterize the set of equilibrium adoption rates delineating the sizes of subscribed traveler populations. The resulting routing strategies are such that all travelers face an identical expected cost and no traveler has the incentive to change her subscription.

==> beliefs.tex <==
%%novalidate
%!TEX root=manuscript.tex
\subsection{Beliefs}\label{sub:belief}
In the framework of Bayesian games \cite{fudenberg1991game}, the notion of ``type'' captures all the private information available to each population (see \cite{harsanyi1967games}). In our model, the private information of each population is the signal it receives from the corresponding TIS, i.e. $\yi$. We define the type of population $\i$ as $\ti$ and the type space as $\Ti$, where for each $\i \in \I$, $\Ti \equiv \Yi$, $\ti \deleq \yi$. Thus, the distribution of type conditional on state is the same as that of signals, i.e. $\psti=\psyi$. Based on type $\ti$, each population generates a belief about the state and the opponent's type, denoted $\muti \in \Delta(\S \times \Tmi)$.

We further assume that the type conditional probability distributions and the prior distribution on states are common knowledge.
\begin{assumption}\label{as:common_knowledge}
The type conditional distribution matrixs, $P^1$, $P^2$ and the prior distribution on states, $\ps(\s)$, are common knowledge of the game. 
\end{assumption}

The beliefs $(\mu^i)_{\i \in \I}$ can be expressed as follows: $\forall \s \in \S, \ti \in \Ti, \tmi \in \Tmi,  \i \in \I.$
\begin{equation}\label{eq:belief_complex}
\begin{split}
\muti&=\frac{\pro^{\i}(\s, \ti, \tmi)}{\pro(\ti)}=\frac{\ps(\s)\pro^{\i}(\ti, \tmi|\s)}{\pro(\ti)}\\
&=\underbrace{\frac{\ps(\s)p(\ti|\s)}{\pro(\ti)}}_{\pro(\s|\ti)} \cdot \pro^{\i}(\tmi|\ti, \s),
\end{split}
\end{equation}
where $\pro^{\i}(\tmi|\ti, \s)$ is population $\i$'s beliefs of the other population's type probability distribution conditional on state $\s$. We know from Assumption \ref{as:independent} that $\ti, \tmi$ are independent conditional on state $\s$. We also know from Assumption \ref{as:common_knowledge} that population $\i$ knows the accuracy matrix of the other population, $P^{-\i}$. Thus, $\pro^{\i}(\tmi|\ti, \s)=p(\tmi|\s)$. We can simplify \eqref{eq:belief_complex} as:
\begin{equation}\label{eq:belief_fun}
\forall \i \in \I, \quad \muti=\frac{\ps(\s)p(\ti|\s)}{\pro(\ti)} \cdot p(\tmi|\s),
\end{equation}
where the marginal distribution $\pro(\ti)$ is in \eqref{eq:marginal_type}. 

When Assumption \ref{as:common_knowledge} is satisfied, there exists common prior, $\pi(\s, \tone, \ttwo) \in \Delta(\S \times \Tone \times \Ttwo)$:
\begin{equation}
\pi(\s, \tone, \ttwo)=\ps(\s) \cdot \pstone \cdot \psttwo.
\end{equation}
Beliefs $\mu^1, \mu^2$ can be restated as the conditional probability derived from the common prior:
\begin{equation}\label{eq:objective_fun}
\muti=\frac{\pi(\s, \ti, \tmi)}{\pro(\ti)}, \quad \forall \s \in \S, \i \in \I, \ti \in \Ti.
\end{equation}



==> equilibrium_cost.tex <==
%%novalidate
\section{Equilibrium Cost}
In this section, we discuss how expected cost of individual commuters of each population, denoted as $\ciwel$, and the expected social average cost, denoted as $\cwesocial$ change with respect to $\lamb$. We know from Corollary \ref{essential_unique} that the BWE is essentially unique in the sense that $\llamb$ is unique for any equilibrium strategy profile. Therefore, both $\ciwel$ and $\cwesocial$ are identical for $\qwelamb$. 

Before discussing the properties of $\ciwel$ and $\cwesocial$, we first prove the continuity and convexity of the optimal-value potential function. This part of discussion follows the discussion in Fiacco \cite[]. We provide a brief review of Fiacco's theory in the Appendix.


We define $\Plamb(\lamb)$ as the optimal value of $\potential$ when $l$ is the equilibrium load distribution of game $\gl$, i.e.:
\begin{equation}\label{Plamb}
\Plamb(\lamb)=\potential(\llamb).
\end{equation}

The next lemma shows that $\Plamb(\lamb)$ is continuous, differentiable and convex in $\lamb$.
\begin{lemma}
$\forall \lamb \in (0,1)$, $\Plamb(\lamb)$ is countinuous and differentiable in $\lamb$. Furthermore, $\Plamb$ is convex in $\lamb$.
\end{lemma}
\begin{proof}
The potential funtion $\potential(q)$ is convex in $q$ and does not change with respect to $\lamb$. Thus, $\potential(q)$ is convex in $(q, \lamb)$. Constraints \eqref{sub:demand} is affine in both $q$ and $\lamb$. Constraints \eqref{sub:positive} is linear, thus convex in $\lamb, q$. The domain of $\lamb$ is $[0,1]$, which is convex. We know from Proposition \ref{continuous_phi} in the Appendix that $\Plamb(\lamb)$ is convex in $\lamb$. 

Since the feasible solution set is closed and convex, $\potential(q)$ is continuous and convex in $q$, the optimal solution is attainable. Therefore, the optimal valued functiom $\Plamb(\lamb)$ is continuous and differentiable in $\lamb$. 
\end{proof}



In the following theorem, we further show that $\Plamb (\lamb)$ has a bathtub shape with respect $\lamb$.  
\begin{theorem}[Bathtub Theorem]\label{bathtub}
\begin{itemize}
\item When $\lamb \in [0, \lambl)$, $\frac{d \Plamb(\lamb)}{d \lamb}<0$.
\item When $\lamb \in [\lamb, \lambup]$, $\frac{d \Plamb(\lamb)}{d \lamb}=0$.
\item When $\lamb \in (\lambup, 1]$, $\frac{d \Plamb(\lamb)}{d \lamb}>0$.
\end{itemize}
\end{theorem}
The name Bathtub Theorem comes from the fact that the function $\Plamb(\lamb)$ is a U-shape function of $\lamb$ with a flat bottom in the range of $[\lambl, \lambup]$.
\begin{proof}
\begin{itemize}
\item  When $\lamb \in \Retwo,$ we know from Theorem \ref{l_behavior} that $\lrwe(\t)=\lrdag(\t), \forall \r \in \R, \t \in \T$. $\Plamb(\lamb)$ is a constant with respect to $\lamb$. Since $\Plamb(\lamb)$ is differentiable, we have $\frac{d \Plamb(\lamb)}{d \lamb}=0, \forall \lamb \in (\lambl, \lambup)$.
\item When $\lamb \in [0, \lambl)$, we first show that the solution of the following optimization problem satisfies \eqref{left_bind}:
\begin{equation}\label{constraint_leq}
\begin{split}
&\min_{l} \quad \potential (l)\\
s.t. \quad &1-\frac{\sum_{\r \in \R} \min_{\tkone \in \Tone} \lr(\tkone, \ttwo_1)}{D} \leq \lamb \\
&\text{$l$ satisfies \eqref{sub:balance}, \eqref{sub:ldemand}, \eqref{sub:l_positive}}.
\end{split}
\end{equation}
The proof by contradiction is the same as that in the proof of Theorem \ref{l_behavior}. Assuming \eqref{left_bind} is not satisfied, then $\lrdag$ is the solution, which violates the assumption that $\lamb < \lambl$. Therefore, the optimal solution of \eqref{constraint_leq} satisfies \eqref{left_bind}. The optimal solution of \eqref{constraint_left} is the same as the optimal solution of \eqref{constraint_leq}. We consider $\forall \lambp, \lamb$ such that $0 \leq \lambp < \lamb < \lambl$. The corresponding equilibrium load distributions $\lrwep$ and $\llambr$ satisfies:
\begin{equation}
1-\frac{\sum_{\r \in \R} \min_{\tkone \in \Tone} \lrwep(\tkone, \ttwo_1)}{D} = \lambp< \lamb =1-\frac{\sum_{\r \in \R} \min_{\tkone \in \Tone} \llambr(\tkone, \ttwo_1)}{D}
\end{equation}

Therefore, $\lrwep$ lies in the feasible set of the optimization program \eqref{constraint_leq} corresponding to $\lamb$, but $\lrwep$ does not satisfy the equation \eqref{left_bind}, so $\lrwep$ is not the optimal solution of \eqref{constraint_leq}. We have:
\begin{equation}
\Plamb(\lambp)>\Plamb(\lamb), \quad \forall \lamb \in [0, \lambl).
\end{equation}
Since we know $\Plamb(\lamb)$ is differentiable, we know that $\frac{d \Plamb(\lamb)}{d \lamb}<0, \forall \lamb \in [0, \lambl)$.
\item Analogously, we know that $\frac{d \Plamb(\lamb)}{d \lamb}>0, \forall \lamb \in (\lambup, 1]$.
\end{itemize}
The theorem is proved by summing up all three cases. 
\end{proof}
Bathtub theorem charaterizes the shape of $\Plamb(\lamb)$. In regime $\Reone$ and $\Rethree$, $\Plamb(\lamb)$ strictly decreasing and strictly increasing respectively. In regime $\Retwo$, $\Plamb(\lamb)$ is constant. This shape first coicides with our observation in Theorem \ref{l_behavior} that in regime $\Retwo$, the equilibrium load distribution is $\lrdag$. In regime $\Reone, \Retwo$, equilibrium load distribution changes as $\lamb$ changes. The result in Bathtub theorem also matches the result that $\Plamb(\lamb)$ is convex in $\lamb$. 




\begin{lemma}\label{unique_lag}
For any given $\lamb \in [0, 1]$, the parametric optimization problem \eqref{q_program} satisfies KKT, LICQ, SOSC conditions at optimal points in all three regimes. The Lagrangian multipliers $\alti, \betir$ are unique and can be expressed as \eqref{alpha_define}, \eqref{beta_define}. SCS holds in regime $\Reone$ and $\Rethree$. $(\qtirlamb, \altilamb, \betirlamb)$ are unique and once continuously differentiable in regime $\Reone, \Rethree$. $\Plamb(\lamb)$ is twice continuously differentiable with respect to $\lamb$ in regime $\Reone, \Rethree$.
\end{lemma}
\begin{proof}
\begin{itemize}
\item Since \eqref{potential_opt} is a convex optimization problem, KKT conditions are satisfied at any optimal points.
\item LICQ holds at equilibrium points.\\
The left hand side of constraints \eqref{sub:demand} are afine functions and the gradients are linearly independent. The left hand side of constraints \eqref{sub:positive} are also affine and the gradients are linearly independent. Assuming LICQ is violated, the constraints of \eqref{sub:positive} that are binding include $\{\qtir\}_{\r \in \R}=0$ for at least one specific $\ti$, which contradicts with the fact that $\sum_{\r \in \R}\qtir=\lamb^i D, \forall \ti \in \Ti, \i \in \I$. Therefore, LICQ is satisfied. We know from Proposition \ref{unique_lagrangian} that the associated Lagrangian multipliers $\alti, \betir$ are unique. In the prove of Theorem \ref{q_opt}, we show by construction that $\alti$, $\betir$ defined as \eqref{alpha_define}, \eqref{beta_define} satisfies KKT conditions, thus are unique Lagrangian multipliers. 
\item SOSC is satisfied. \\
For any direction $z$ that satisfies constraints \eqref{z_constraint}, since $\nabla_{q} \qtir$ has 1 on the position corresponding to $\qtir$ and 0 on others, we know from \eqref{sub:g_gradient} that $z$ is non-negative. \eqref{sub:h_gradient} requires $z$ to be zero. Therefore, non-zero $z$ does not exist, any equilibrium points satsifies SOSC condition.
\item We now prove that SCS holds in regime $\Reone, \Rethree$ by contradiction. If SCS does not hold in regime $\Reone$, with out loss of generality, we assume that there exist $\lamb_1 \in \Reone, \tkone, \r_1$ such that $q_{r_1}(\tkone, \lamb_1)=0$ and $\beta^{\tkone}_{r_1}(\lamb_1)=0$. Recall from the expression of $\beta_{r_1}^{\tkone}(\lamb_1)$ from \eqref{beta_define}, we have: 
\begin{equation}
\begin{split}
q_{r_1}(\tkone, \lamb_1)&=0\\
\beta_{r_1}^{\tkone}(\lamb_1)&=Pr(\tkone)\mathbb{E}[c_{r_1}(l_{r_1}(\qwe_{\lamb_1}))|\tkone]-\min_{\r \in \R} Pr(\tkone)\mathbb{E}[c_r(\lr(\qwe_{\lamb_1}))|\tone]=0.
\end{split}
\end{equation}
Let $\epsilon$ be a sufficient small positive number, for $\lamb=\lamb+\epsilon$, we construct strategy for population 1  and 2 as $q^1(\lamb), q^2(\lamb)$, where:
\end{itemize}
\end{proof}

%====individual cost=====
We next calculate the first order derivative of $\Plamb(\lamb)$ with respect to $\lamb$ and show the link between derivative and $\ciwel$. 
\begin{theorem}
We can write the first order derivative of $\Plamb(\lamb)$ as the difference of the expected cost of individual commuters in each populations as follows:
\begin{equation}\label{gradient_difference}
\frac{d \Plamb(\lamb)}{d \lamb}=(\conewel-\ctwowel)D.
\end{equation}
Furthermore, 
\begin{itemize}
\item $\forall \lamb \in [0, \lambl)$, $\conewel<\ctwowel$.
\item $\forall \lamb \in [\lambl, \lambup]$, $\conewel=\ctwowel$.
\item $\forall \lamb \in (\lambup, 1]$, $\conewel>\ctwowel$.
\end{itemize}
\end{theorem}


\begin{proof}
 Recall that the Lagrangian function of \eqref{potential_opt} is \eqref{lagrangian}, where the Lagrangian multipliers are $\betir \geq 0, \forall \ti \in \Ti, \i \in \I, \r \in \R$ and $\alti, \forall \ti \in \Ti, \i \in \I$. We know from proposition \ref{} in the appendix that the Lagrangian multipliers are unique when LICQ is satisfied at equilibrium point. Thus the Lagrangian multiplier is unique, and can be expressed as \eqref{alpha_define}, \eqref{beta_define}. 
Fiacco points out in Proposition \ref{} that when the optimal valued function $\Plamb(\lamb)$ is differentiable with respect to $\lamb$, the derivative can be written as:
\begin{equation}\label{gradient_original}
\frac{d \Plamb(\lamb)}{d \lamb} = \min_{\qwelamb} \max_{(\alpha^{*}, \beta^{*})} \frac{\partial L(q, \alpha, \beta)}{\partial \lamb}.
\end{equation}
Since the Lagrangian multipliers at equilibrium is unique, we can simplify the first order derivative from \eqref{gradient_original} as:
\begin{equation}
\frac{d \Plamb(\lamb)}{d \lamb} = \min_{\qwelamb}\frac{\partial L(q, \alpha, \beta)}{\partial \lamb}
\end{equation}
We calculate $\frac{\partial L(q, \alpha, \beta)}{\partial \lamb}$ as:
\begin{equation}\label{l_lamb_partial}
\frac{\partial L(q, \alpha, \beta)}{\partial \lamb}=\min_{\qwelamb} (\sum_{\tone \in \Tone} \alpha^{\tone}(\qwelamb)-\sum_{\ttwo \in \Ttwo} \alpha^{\ttwo}(\qwelamb)) D
\end{equation}
Put the expression of Lagrangian multipliers in, we further simplify the first order derivative as:
\begin{equation}
\frac{d \Plamb(\lamb)}{d \lamb} = \min_{\qwelamb}(\sum_{\tone \in \Tone}\min_{\r \in \R}Pr(\tone) \ecrtonewelamb- \sum_{\ttwo \in \Ttwo}\min_{\r \in \R}Pr(\ttwo) \ecrttwowelamb) D
\end{equation}
Since $\ecrtonewelamb, \ecrttwowelamb$ are functions of equilibrium load distribution, they are identical for any equilibrium strategy profile. Recall the expressions of $\ecrti$ from \eqref{ecrti}, we get:
\begin{equation}
\begin{split}
\frac{d \Plamb(\lamb)}{d \lamb} &= (\sum_{\tone \in \Tone}\min_{\r \in \R} \sum_{\s \in \S} \sum_{\ttwo \in \Ttwo}\pi\left(\s, \tone, \ttwo\right) \crsfun\left(\llambr(\tone, \ttwo)\right)\\
&-\sum_{\ttwo \in \Ttwo} \min_{\r \in \R} \sum_{\s \in \S} \sum_{\tone \in \Tone} \pi\left(\s, \tone, \ttwo\right) \crsfun\left(\llambr(\tone, \ttwo)\right)) D
\end{split}
\end{equation}
Recall the expression of $\ctiwel$ and $\ciwel$ from \eqref{ctiwel} and \eqref{ciwel}, and since at BWE, $\qwe$ only put positive demand on routes which have the minimum expected travel time, $\ctiwel$ can be restated as:
\begin{equation}
\ctiwel=\min_{\r \in \R} \sum_{\s \in \S} \sum_{\tmi \in \Tmi} \muti \crsfun \left(\lrwe\left(\ti, \tmi \right) \right)
\end{equation}
We can have the expressions for $\ciwel$ in the same way:
\begin{equation}\label{restate_ciwel}
\ciwel=\sum_{\ti \in \Ti} \min_{\r \in \R} \sum_{\s \in \S} \sum_{\tmi \in \Tmi} \pi(\s, \ti, \tmi) \crsfun \left(\lrwe\left(\ti, \tmi \right) \right)
\end{equation}
We can see that:
\[\frac{d \Plamb(\lamb)}{d \lamb}=(\conewel-\ctwowel)D\]
which is \eqref{gradient_difference}. Following from Theorem \ref{bathtub}, we immediately get that population 1 has lower averge cost in regime $\Reone$. Population 2 has lower average cost in regime $\Rethree$. Two populations have the same average cost in regime $\Retwo$.
\end{proof}


The following proposition shows a simple case in which $\lambup=1$, thus $\Plamb(\lamb)$ first decreases then remain constant with respect to $\lamb$. 

\begin{proposition}\label{no_info}
If population 2 gets no information from the signal. i.e. $p^2(t^2|s)=p^2(t^2)$, $\lambup=1$.
\end{proposition}
\begin{proof}
When $p^2(t^2|s)=p^2(t^2)$, $\mu(\s, \tone|\ttwo)$ is identical for any $\ttwo$. Therefore, the strategy of population 2 is identical for any $\ttwo$. $\forall \tktwo, \tktwo \in \Ttwo, \forall \r \in \R$, $\lrdag(\tone_1, \tktwo)=\lrdag(\tone_1, \tktwo)$. Therefore, $\lambup=1$.
\end{proof}


==> figures.tex <==
%%novalidate







%\begin{figure}[H]
% \begin{subfigure}[b]{0.48\textwidth}
% \includegraphics[width=\textwidth]{social_lower.eps}
%       \caption{}
%       \label{fig:soc_8_6_18_20_2}
%    \end{subfigure}
%~
%	\begin{subfigure}[b]{0.48\textwidth}
%	\includegraphics[width=\textwidth]{social_both_inf.eps}
%        \caption{}
%        \label{fig:soc_8_6_18_18_2}
%    \end{subfigure}
%\caption{Equilibrium average cost $\clamb$ bounded by $\copt$.}
%    \end{figure}

==> modelsa.tex <==
%%novalidate
%!TEX root=manuscript.tex
\section{Value of Information in Bayesian Congestion Games}\label{motivate}
Consider a network of two parallel routes, denoted $\rone$ and $\rtwo$. The network state belongs to the set $\S=\{\a, \n\}$, where the state $\a$ represents an incident on $\rone$, and the state $\n$ represents the nominal condition, see Fig. \ref{two_route}. The state $\a$ occurs with probability $p$. The route cost functions are defined as follows: 
\vspace{-5mm}
\begin{multicols}{2}
\begin{equation*}\label{affine_cost}
\begin{split}
\cones(\lone)&=\left\{
\begin{array}{ll}
\aonea \lone +\bone, & \s=\a,\\
\aonen \lone +\bone, & \s=\n.
\end{array}
\right.\\
\ctwo(\ltwo)&=\atwo \ltwo+\btwo,
\end{split}
\end{equation*}
\columnbreak
\begin{figure}[H]
\centering
\includegraphics[width=0.8 \linewidth]{network1.jpg}
\caption{Two Route Network.}
\label{two_route}
\end{figure}
\end{multicols}
\vspace{-7mm}
where $\l_\r$ is the flow through route $\r$. For simplicity, we assume that $\aonen<\atwo <\aonea$ and $\bone=\btwo\deleq b$.  The network faces a unit demand comprising of two traveler populations: population 1 with demand $\lamb^1$ and population 2 with demand $\lamb^2=1-\lamb^1$. Each population $\i \in \I=\{1,2\}$ receives a noisy observation (signal) $\ti$ of the network state from its information system. Thus, the signal space of population $\i$ is $\Ti=\{\a, \n\}$. 
We assume that population 1 receives the correct state with probability 1 (i.e. complete information), and population 2 receives signal $\a$ or $\n$ with probability $0.5$, independent of the state (i.e. no information); this information structure is common knowledge. 

Let $\qi_1(\ti)$ denote the demand assigned to $\rone$ by population $\i$ when receiving signal $\ti$; the remaining demand $\(\lamb^i-\qi_1(\ti)\)$ is assigned to $\rtwo$. Since signal $\ttwo$ is independent of the state, we have $\qtwo_1(\a)=\qtwo_1(\n) \deleq \qtwo_1$. Any feasible demand assignment must satisfy the constraints: $0 \leq \qone_1(\tone) \leq \lamb^1 $ and $0 \leq \qtwo_1 \leq \lamb^2$. We represent a feasible strategy profile as $q_1=\(\qone_1(\a), \qone_1(\n), \qtwo_1\)$. 

The expected route cost on $\r$ for population 1 receiving signal $\tone$, denoted $\ecrtone$, can be expressed as follows: 
\vspace{-5mm}
\begin{align*}
\econeh&=\left\{
\begin{array}{ll}
\conea \(\qone_1(\a)+\qtwo_1\), \quad & \tone=\a,\\
\conen \(\qone_1(\n)+\qtwo_1\), \quad & \tone=\n.
\end{array}
\right.\\
\ectwoh&=\ctwo (1 -\qone_1(\tone)-\qtwo_1), \quad \forall \tone \in \Tone.
\end{align*}
For population 2, the expected route costs $\ecrttwo$ can be expressed as:
\begin{align*}
\econel&=p \cdot \conea\(\qone_1(\a)+\qtwo_1\)+ (1-p) \cdot \conen \(\qone_1(\n)+\qtwo_1)\),\\
\ectwol&=p \cdot \ctwo ( 1-\qone_1(\a)-\qtwo_1)+(1-p) \cdot \ctwo ( 1-\qone_1(\n)-\qtwo_1).
\end{align*}
This routing game with heterogeneously informed populations admits a Bayesian Wardrop equilibrium as defined in Sec. \ref{sub:game}. Let $\qwe_1=\(\qweone_1(\a), \qweone_1(\n), \qwetwo_1 \)$ denote an equilibrium. Note that each population - given the signal it receives - assigns all the demand on one route, or splits on both routes. Thus, there are $3\times 3 \times 3=27$ possible cases. Our results enable us to study how the equilibrium strategies and route flows change as the population size $\lamb^1$ varies from 0 to 1. 


In particular, there exists a threshold $0 \leq \lambl \leq 1$ of population 1's demand, which distinguishes two equilibrium regimes, i.e. the equilibrium structure is different depending on whether $\lamb^1 \in [0, \lambl)$ or $\lamb^1 \in [\lambl, 1]$. For this example, we have $\lambl&\deleq \atwo\(\frac{1}{\aonen+\atwo} -\frac{1}{\aonea+\atwo}\)$.

In the first regime, i.e. if $\lamb^1 \in [0, \lambl)$, the game admits a unique equilibrium:
\vspace{-3mm}
\begin{align*}
 \qweone_1(\a)&=0 \notag\\
 \qweone_1(\mathbf{n})&=\lamb^1 \notag\\
 \qwetwo_1&=\frac{\atwo}{\abar+\atwo}-\lamb^1\frac{(1-p) (\aonen+\atwo)}{\abar+\atwo}\notag
\end{align*}
where $\abar=p\aonea+(1-p)\aonen$. This regime corresponds to the following case:
\[\mathbb{E}[c_1(\qwe)|\a] >\mathbb{E}[c_2(\qwe)|\a], \quad \mathbb{E}[c_1(\qwe)|\n] <\mathbb{E}[c_2(\qwe)|\n],  \quad \mathbb{E}[c_1(\qwe)|\ttwo] =\mathbb{E}[c_2(\qwe)|\ttwo].\]
Thus, in equilibrium, population 1 faces different route costs on each route. In particular, in state $\n$ (state $\a$), population 1 assigns all its demand on route $\rone$ (resp. route $\rtwo$), and population 2 splits its demand on both routes. The induced equilibrium flow on $\rone$ is given by: $\l_1^{*}(\tone, \ttwo)=\qwetwo$ if $\tone=\a$, and $\l_1^{*}(\tone, \ttwo)=\lamb^1+\qwetwo$ if $\tone=\n$. 


In the second regime, i.e. if $\lamb^1 \in [\lambl, 1]$, the set of equilibria can be represented as follows:
\vspace{-3mm}
\begin{equation*}\label{eq:q_two}
\begin{split}
 \qweone_1(\a)&=\chi\\
 \qweone_1(\mathbf{n})&=\lambl+\chi\\
 \qwetwo_1&=\frac{\atwo}{\aonea+\atwo}-\chi,
\end{split}
\end{equation*}
where $\max \left\{0, \lamb^1 -\frac{\aonea}{\aonea +\atwo}\right\} \leq \chi \leq \min \left\{\frac{\atwo}{\aonea+\atwo}, \lamb^1  -\lambl  \right\}$. Note that the equilibrium set is a connected set for $\lamb^1 \in (\lambl, 1)$ and singleton set for $\lamb^1=\lambl$ or $\lamb^1=1$, the equilibrium is unique. Any equilibrium in this regime satisfies:
\[\mathbb{E}[c_1(\qwe)|\a] =\mathbb{E}[c_2(\qwe)|\a], \quad \mathbb{E}[c_1(\qwe)|\n] =\mathbb{E}[c_2(\qwe)|\n], \quad \mathbb{E}[c_1(\qwe)|\ttwo] =\mathbb{E}[c_2(\qwe)|\ttwo],\]
i.e. each population faces equal route costs. Consequently, each population splits its demand on both routes. Furthermore, all equilibria induce a unique route flow that is independent of $\lamb$: $\l_1^*(\tone, \ttwo)=\frac{\atwo}{\aonea+\atwo}$ if $\tone=\a$, and $
\l_1^*(\tone, \ttwo)=\frac{\atwo}{\aonen+\atwo}$ if $\tone=\n$. 

Notice that if $\lamb^1 \in [0, \lambl)$, we have $\q_1^{*1}(\n)-\qweone_1(\a)=\lamb^1$, i.e. population 1 shift all its demand from $\rone$ to $\rtwo$ on receiving incident information. However, if $\lamb^1 \in [\lambl, 1]$, we have $\q_1^{*1}(\n)-\qweone_1(\a)=\lambl\leq \lamb^1$, i.e. information only influences part of population 1's demand. In other words, information maximally impacts population 1 in the first regime, and only partially in the second regime. 

Now, we can calculate the expected equilibrium costs, denoted $\cilamb$. If $\lamb^1 \in [0, \lambl)$, $\conelamb$ can be written as follows:
\begin{align*}
\conelamb&=p \ectwoha + (1-p) \econehn \notag =b+\bar{C}+\bar{C}^1 \lamb^1\\
\ctwolamb&=\econel =\ectwol \notag =b+\bar{C}+\bar{C}^2\lamb^2,
\end{align*}
where 
\vspace{-3mm}
\begin{align*}
\bar{C}&=\frac{\atwo(\aonen(1-p^2)+\aonea p^2)}{\abar+\atwo},\\
\bar{C}^1&=\frac{p(1-p)\aonen(\aonea+\atwo)+p(1-p)\atwo(\aonen+\atwo)}{\abar+\atwo},\\
\bar{C}^2&=\frac{\atwo p(1-p)(\aonea-\aonen)}{\abar+\atwo}.
\end{align*}
Since $\ctwolamb-\conelamb=\bar{C}^2 \lamb^2-\bar{C}^1\lamb^1>0$, population 1 gains by receiving information in comparison to population 2 which is uninformed. Furthermore, $\lambl$ is the threshold size of population 1 at which this gain becomes 0.


On the other hand, if $\lamb^1 \in [\lambl, 1]$, the expected cost of both populations are identical in equilibrium, because each population faces equal route costs:
\begin{align*}
\conelamb=\ctwolamb=b+\bar{C}+\frac{\bar{C}^1 \bar{C}^2}{\bar{C}^1+\bar{C}^2}.
\end{align*}
The relative value of information $\rvlamb$, which is the difference of two population costs in equilibrium can be obtained as follows:
\begin{align*}
\rvlamb&\deleq \ctwolamb-\conelamb
=\left\{
\begin{array}{ll}
\frac{1}{\abar+\atwo} p\(1-p\)\left[\atwo(\aonea-\aonen)-\lamb^1(\aonea+\atwo)(\aonen+\atwo)\right], & \quad \lamb^1 \in [0, \lambl),\\
0, & \quad \lamb^1 \in [\lambl, 1].
\end{array}
\right.
\end{align*}
Thus, $\rvlamb$ monotonically decreases in the first regime, and remains 0 in the second regime. 

Finally, the equilibrium average cost is simply the average expected cost in equilibrium:
\vspace{-3mm}
\begin{align*}
\clamb=\lamb^1 \conelamb+\lamb^2 \ctwolamb
=\left\{
\begin{array}{ll}
\(\bar{C}^1+\bar{C}^2\)(\lamb^1)^2-2 \bar{C}^2\ \lamb^1+\bar{C}+b+\bar{C}^2, & \quad \forall \lamb^1 \in [0, \lambl),\\
b+\bar{C}+\frac{\bar{C}^1 \bar{C}^2}{\bar{C}^1+\bar{C}^2}, & \quad \forall \lamb^1 \in [\lambl, 1].
\end{array}
\right.
\end{align*}
Note that $\clamb$ monotonically decreases with $\lamb^1$ in the first regime, and attains a fixed (minimum) value in the second regime. To see this, for $\lamb^1 \in [0, \lambl)$, we can write:
\begin{align*}
\frac{\partial \clamb}{\partial \lamb^1}=2 \(\bar{C}^1+\bar{C}^2\) \lamb^1 - 2\bar{C}^2<0,
\end{align*}
and thus $\frac{\partial \clamb}{\partial \lamb^1}=0$ when $\lamb^1=\lambl$. Thus, increasing the size of informed population decreases the average cost but only when it is below $\lambl$. 

We illustrate the aforementioned results using the following parameters: $\aonen=1$, $\aonea=3$, $\atwo=2$, $b=20$, and $p=0.2$. Fig. \ref{fig:H_75_L_50_D_1_stra} shows the equilibrium strategy $\(\qweone_1(\a), \qweone_1(\n), \qwetwo_1 \)$, the flow through route $\rone$ in each state, and also the expected population costs and average cost in equilibrium. The costs are normalized by the socially optimum cost, denoted $C^{so}$, which is the minimum cost achievable by a fully informed social planner, averaged over both states. 
\begin{figure}[h!]
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{strategy.eps}
        \caption{}
        \label{fig:H_100_L_50_D_1_q}
    \end{subfigure}
~
\centering
	\begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{flow.eps}
        \caption{}
        \label{fig:H_100_L_50_D_1_f}
    \end{subfigure}\\
   \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{ind_mot.eps}
        \caption{}
        \label{fig:H_100_L_50_D_1_p}
    \end{subfigure}
~
\centering
	\begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{social.eps}
        \caption{}
        \label{fig:H_100_L_50_D_1_s}
    \end{subfigure}
    \caption{(a) Equilibrium strategies; (b) Equilibrium route flows;\\
     (c) Equilibrium population costs; (d) Equilibrium average cost.}
    \label{fig:H_75_L_50_D_1_stra}
\end{figure}
For this simple example, we evaluated the effect of varying $\lamb^1$ on the equilibrium structure, population costs and average cost in equilibrium. 




==> optimization.tex <==
%%novalidate
%!TEX root = revision_two.tex
\color{red}
\section{Extensions and discussions}\label{sec:optimization}
In this section, we discuss the extension of our results when the following model aspects are included: non-decreasing edge cost functions, networks with multiple origin-destination pairs, and TISs which minimize the cost of subscribed populations.

\noindent \emph{Non-decreasing edge cost functions.}
    Our results hold in games where the edge costs are non-decreasing (rather than strictly increasing) in the edge loads. In particular, such a game still admits the same weighted potential function as in \eqref{eq:potential_q}, although now the essential uniqueness only applies to the equilibrium edge costs, rather than the loads. All results in Secs. \ref{equilibrium_regime} and \ref{sec:general_cost} remain unchanged for non-decreasing cost functions. However, under pairwise perturbation of size vector, the edge load vector $\wdagij$ induced by the optimal flow vectors of \eqref{eq:basic_opt_ij} is no longer unique.
    Therefore, each regime threshold as in \eqref{pairwise_threshold} is the optimal solution of a bi-level optimization problem, which is more complicated from a computational viewpoint.
    
\noindent \emph{Networks with multiple origin-destination pairs.}
    Consider a network with the set of origin-destination (o-d) pairs $\K$, where each o-d pair $k \in \K$ is connected by a set of routes $\R_k$. The demand of travelers between each o-d pair $k \in \K$ is $D_k > 0$, and the fraction of travelers between o-d pair $k$ who subscribe to TIS $i \in \I$ is $\lambda_k^i$. In equilibrium, travelers between each o-d pair choose routes with the minimum expected cost among all routes between that o-d pair. 
    
    Equation \eqref{eq:potential_q} is still the weighted potential function of the game, and hence Theorem \ref{q_opt} still holds. Propositions \ref{Lprime} and \ref{l_opt} hold with simple modifications: the demand constraint \eqref{sub:ldemand} is satisfied for each $k \in \K$, i.e. $\sum_{\r \in \R_k} f_r(\t)=\D_k$, and the information impact constraint \eqref{sub:popu_i} is satisfied for each $k \in \K$ and $\i \in \I$, i.e. $
D_k  - \sum_{r \in \R_k} \min_{t^i \in \T^i} f_{r}(t^i, t^{-i}) \leq \lambda_k^i \D_k$.   

All the results on qualitative properties of equilibrium structure, relative ordering of average costs of travelers, and adoption rates remain unchanged for travelers between each o-d pair. In particular, for any $k \in \K$ and any $\i, \j \in \I$, when perturbing the sizes $\lamb_k^i$ and $\lamb_k^j$, three regimes (one or two may be empty) can be distinguished by whether or not the information impacts all the travelers between o-d pair $k$ who subscribe to TIS $i$ (resp. $j$).
Moreover, by analogously applying sensitivity analysis, we show that the relative value of information, now defined as the travel cost saving experienced by travelers between o-d pair $k$ who subscribe to TIS $i$ compared with travelers who subscribe to TIS $j$, is positive, zero, and negative in the three regimes respectively. 
We also analyze how travelers between each o-d pair $k \in \K$ choose TIS subscription. We note that the relative value of information and adoption rates for travelers between one o-d pair depends on the sizes and the route choices of populations between the same o-d pair as well as between other o-d pairs. This is because travelers between different o-d pairs may take common routes and edges, and hence impact each other’s costs. 
    
\noindent \emph{Cost minimizing TISs.} Our analysis approach and results can be instantiated to a modified game, where each TIS aims at minimizing the total cost of their subscribed traveler population based on the private information of the unknown state. That is, in the modified game, the players are the TISs (instead of the traveler populations in the original game), who send direct routing recommendations to their subscribed travelers based on the heterogeneous information of the unknown state. Travelers are not strategic, and always follow the recommended routes even though the costs of these routes may not be the minimum. To distinguish the modified game from the original game, we denote the strategy profile in the modified game as $\tilde{q}$, and the load vector as $\tilde{w}$.


In equilibrium, the routing strategy of TIS $\i$ with type $\ti$ minimizes the total cost of population $i$ based on the private belief and the strategies of all other TISs, i.e. \begin{align}\label{eq:opt_i}
\tilde{\q}^{\i*}(\ti) \in \argmin_{\tilde{\q}^i(\ti)} \sum_{\s \in \S} \sum_{\tmi \in \Tmi} \muti \sum_{\r \in \R} \(\sum_{\e \in \r} \cesfun(\tilde{w}_e(\ti, \tmi))\) \tilde{\q}^{\i}_\r(\ti), \quad \forall \i \in \I, \quad \forall \ti \in \Ti,
\end{align}
where $\tilde{w}_e(\ti, \tmi)= \sum_{\r \ni \e} \(\sum_{\j \in \I \setminus \{\i\}}\tilde{\q}^{j*}_r(\tj)+ \tilde{\q}^{\i}_\r(\ti)\)$ is the aggregate edge load on edge $\e$. 

We now show that the equilibrium strategy profile can be solved by an optimization problem. To ensure the uniqueness of the equilibrium load vector, we assume that the total cost of each edge $\we \cesfun(\we)$ is strictly convex in $\we$ for all $\e \in \E$ and all $\s \in \S$. 
\begin{proposition}\label{prop:modified}
A strategy profile $\tilde{q}^{*} \in \Q(\lamb)$ is an equilibrium strategy profile of the modified game if and only if it minimizes the expected total cost of all travelers:
\begin{equation}\label{eq:modified_potential}
\min \quad \mathbb{E}[C(\tilde{q})] \deleq \sum_{\s \in \S} \sum_{\t \in \T} \sum_{\e \in \E} \pi(\s, \t) \tilde{w}_e(\t) \cdot \cesfun(\tilde{w}_e(\t)), \quad s.t. \quad \tilde{q} \in \Q(\lamb),
\end{equation}
where $\tilde{w}(\t)$ is the induced load vector, and $\Q(\lamb)$ is the set of feasible strategy profiles. The equilibrium edge load vector $\tilde{w}^{*}(\lamb)$ is unique.
% \begin{align*}
%     \\
%     =&
% \end{align*}
\end{proposition}

\proof{Proof of Proposition \ref{prop:modified}.} First, we compute the first order derivative of $\mathbb{E}[C(\tilde{q})]$ with respect to $\tilde{q}_r^i(\ti)$ as follows: 
\begin{align}\label{eq:derivative}
    \frac{\mathbb{E}[C(\tilde{q})] }{\partial \tilde{\q}_{\r}^i(\ti)}= \sum_{\s \in \S} \sum_{\tmi \in \Tmi} \sum_{\e \in \r} \pi(\s, \ti, \tmi) \(\cesfun(\tilde{w}_e(\ti, \tmi))+ \tilde{w}_e(\ti, \tmi) \frac{d \cesfun(\tilde{w}_e(\ti, \tmi))}{d \tilde{w}_e(\ti, \tmi)}\)
\end{align}
We define a modified cost function $\tilde{c}_e^s\(\tilde{w}_e\(\ti, \tmi\)\) \deleq \cesfun(\tilde{w}_e(\ti, \tmi))+ \tilde{w}_e(\ti, \tmi) \frac{d \cesfun(\tilde{w}_e(\ti, \tmi))}{d \tilde{w}_e(\ti, \tmi)}$ for all $\e \in \E$ and all $\s \in \S$. Hence, the first-order derivative in \eqref{eq:derivative} equals to the expected cost of route $\r\in \R$ as in \eqref{eq:ecrti}, but with the modified cost function, i.e.  $\frac{\mathbb{E}[C(\tilde{q})] }{\partial \tilde{\q}_{\r}^i(\ti)}= \mathbb{E}[\tilde{c}_r(\tilde{\q})|\ti]$. 

Next, since for any $\e \in \E$, $\t \in \T$, and $\s \in \S$, $\tilde{w}_e(\t) \cdot \cesfun(\tilde{w}_e(\t))$ is strictly convex in $\we(\t)$, analogous to Lemma \ref{lemma:potential_convex}, we know that the objective function $\mathbb{E}[C(\q)]$ in \eqref{eq:modified_potential} is convex in $\q$. Then, analogous to the proof of Theorem \ref{q_opt}, we know that a strategy profile $\tilde{q}$ is an optimal solution of \eqref{eq:modified_potential} if and only if $\tilde{\q}$ satisfies the following condition:
\begin{align}\label{eq:modified_eq}
    \forall \r \in\R, \quad  \tilde{q}_r^i(\ti)>0, \quad \Rightarrow \quad \mathbb{E}[\tilde{c}_r(\tilde{\q})|\ti] \leq \mathbb{E}[\tilde{c}_{r'}(\tilde{\q})|\ti], \quad \forall \r' \in \R, \quad \forall \i \in \I, \quad \forall \ti \in \Ti.
\end{align}
Therefore, to prove Proposition \ref{prop:modified}, it remains to show that for any $\i \in \I$ and any $\ti \in \Ti$, $\tilde{\q}^i(\ti)$ minimizes the expected cost of population $\i$ as in \eqref{eq:opt_i} if and only if it satisfies the condition in \eqref{eq:modified_eq}. Since $\tilde{\q}$ satisfies the feasibility constraint in \eqref{eq:feasible_q}, we can write the Lagrangian of \eqref{eq:opt_i} as follows: 
\begin{align*}
    \tilde{\mathcal{L}}(\tilde{q}^i(\ti), \altitil, \betirtil)=& \sum_{\s \in \S} \sum_{\tmi \in \Tmi} \muti \sum_{\r \in \R} \(\sum_{\e \in \r} \cesfun(\tilde{w}_e(\ti, \tmi))\) \tilde{\q}^{\i}_\r(\ti) \\
    &+ \altitil \(\lambi \D - \sum_{\r \in \R} \tilde{\q}_r^{\i}(\ti)\) - \sum_{\r \in \R} \betirtil \tilde{\q}_r^i(\ti).
\end{align*}
and the set of KKT conditions for the optimal solution as follows: 
\begin{subequations}
\begin{align}
    \frac{\partial \tilde{\lag}}{\partial \tilde{q}_r^i(\ti)} &=  \sum_{\s \in \S} \sum_{\tmi \in \Tmi} \muti\( \sum_{\e \in \r} \cesfun(\tilde{w}_e(\ti, \tmi))\)-\altitil - \betirtil =0, \quad &\forall \r \in \R, \\%\quad \forall \ti \in \Ti, \quad \forall \i \in \I, \label{first_order}\\
\betirtil \tilde{q}_r^i(\ti) &= 0, \quad &\forall \r \in \R, \\%\quad \forall \ti \in \Ti, \quad \forall \i \in \I, \label{com_slack}\\
\betirtil &\geq 0, \quad &\forall \r \in \R. %\quad \forall \ti \in \Ti, \quad \forall \i \in \I. \label{beta_positive}
\end{align}
\end{subequations}
Then, a strategy profile $\tilde{\q}^{*}$ is the optimal solution of \eqref{eq:modified_potential} if and only if 
\hfill \Halmos
\endproof

Proposition \ref{prop:modified} shows that 

Note that the expected cost function $\mathbb{E}[C(\tilde{q})]$ can be viewed as the potential function of the modified game. Moreover, we can re-express $\mathbb{E}[C(\tilde{q})]$ as follows:
\begin{align*}
    \mathbb{E}[C(\tilde{q})]= \sum_{\s \in \S} \sum_{\t \in \T} \sum_{\e \in \E} \pi(\s, \t) \int_{0}^{\sum_{\r \ni \e} \sum_{\i \in \I} \tilde{\q}^{\i}_\r(\ti)} \(\cesfun(z) + z \cdot \frac{d \cesfun(z)}{d z}\) dz.
\end{align*}
That is, the potential function of the modified game can be obtained from the potential function $\Phi(\tilde{q})$ of the original game as in \eqref{eq:potential_q} by substituting the original cost function $\cesfun(\tilde{w}_e)$ with the total marginal cost function $\frac{d \(\tilde{w}_e \cdot \cesfun(\tilde{w}_e)\)}{d \tilde{w}_e} = \cesfun(\tilde{w}_e)+ \we \cdot \frac{d \cesfun(\tilde{w}_e)}{d \tilde{w}_e}$ for all $\e \in \E$ and all $\s \in \S$. Therefore, in equilibrium, travelers take routes with the minimum marginal cost (instead of the original cost function), which leads to minimizing the expected total cost of all travelers. 


Following the same approach as in Secs. \ref{Sec:potential_game} -- \ref{equilibrium_regime}, we characterize the three regimes induced by the perturbation of relative sizes of any pair of populations, and compare the average costs of the perturbed populations in each regime. The values of the regime boundaries given by \eqref{pairwise_threshold} in the modified game will be different from that in the original game since we use a modified potential game as in \eqref{eq:modified_potential}. Furthermore, analogous to Sec. \ref{sec:general_cost}, we characterize the set of population sizes $\tilde{\Lambda}^{\dagger}$, where the value of the potential function in equilibrium is the minimum across all $\lamb$, and all travelers experience the same average costs in equilibrium. Interestingly, since the potential function in the modified game is the expected total cost of all travelers, the impact of $\lamb$ on the value of potential function is equivalent to the impact on the equilibrium cost of all travelers. Therefore, we can conclude that the total cost of all travelers is minimized when $\lamb \in \tilde{\Lambda}^{\dagger}$. 

\color{black}
 





==> social_value.tex <==
%%novalidate
\subsection{Equilibrium Inefficiency}\label{social_value}
Finally, we relate our work to the well-known result of \cite{roughgarden2012price} on inefficiency due to selfish routing. We first define a benchmark to compare to the equilibrium average cost as defined in \eqref{eq:average_cost_def}. Given any feasible strategy profile $\q \in \Q(\lamb)$, we denote the average cost of all travelers as $C(\q)\deleq \frac{1}{\D} \sum_{\i \in \I}\sum_{\ti \in \Ti} \pro(\ti) \sum_{\r \in \R} \ecrti \qtir$. For any feasible size vector $\lamb$, we define $\copt$ as the minimum average cost over all feasible strategy profiles:
\begin{align}\label{copt}
\copt \deleq\min_{\q \in \Q(\lamb)} C(\q).
\end{align} 
Let $\qopt$ denote a feasible strategy that attains the minimum average cost. It is clear that $\copt$ is a trivial lower bound of $\clamb$ for any size vector $\lamb$. 

The cost $\copt$ can be seen as the average cost minimized by an ``informationally constrained'' social planner who routes the demand of each population $\i \in \I$ according to $\q^{\i,opt}$ based on the population's private signal, but not knowing the network state or signals received by the other populations. Therefore, the benchmark $\copt$ is the minimum average cost in the same asymmetric information environment as the game $\game$, and the inefficiency caused by the selfish routing can be evaluated by the ratio $\clamb /\copt$. By straightforward extension of the well-known result in \citet{roughgarden2004bounding} on the worst-case inefficiency in complete information congestion games, we obtain a tight upper bound of $\clamb/\copt$ in our information environment for any size vector $\lamb$, see Proposition \ref{pigou_bound}. 

Note that one can consider socially optimal cost, denoted $\cso$, as an alternative benchmark to $\copt$. As defined in \eqref{cso_def}, $C^{so}$ is the minimum average cost achieved by a fully informed social planner, i.e. the one who knows the true state and seeks to minimize the average cost over all nature states. Clearly, given any size vector $\lamb$, $\cso \leq \copt \leq \clamb$. This ratio $\clamb/\cso$ represents the combined loss of efficiency due to selfish routing as well as information incompleteness about the network state. In general, the ratio is hard to analyze due to the complexity of heterogeneous information environment; see \cite{roughgarden2012price} for conditions under which this ratio can be analyzed. However, since our focus is on evaluating the inefficiency due to selfish routing, we simply adopt $\copt$ as our benchmark. 

The next proposition provides a condition on the edge cost functions for which there is no inefficiency due to selfish routing, and consequently, one achieves a stable socially fair, and efficient outcome when $\lamb \in \Lambdag$.

 
\begin{proposition}\label{homo_bathtub}
For any $\s \in \S$ and any $\e \in \E$, if the edge cost functions in game $\game$ can be written as $\cesfun(\we)=h_e^s(\we)+b_e^s$, where $h_\e^\s$ is a homogeneous function with degree $k>1$, and $\{b_e^s\}_{\e \in \E, \s \in \S}$ satisfies $\sum_{\e \in \r} b_e^s =b^\s$, for any $\s \in \S$, and any $\r \in \R$, then $\frac{\clamb}{\copt}=1$ for any size vector $\lamb$. Furthermore, the minimum of the equilibrium average cost $\clamb$ is achieved in the set $\Lambdag$, i.e. $\Lambdag= \argmin_{\lamb} \clamb$. 
\end{proposition}
The sufficient condition for this result restricts the edge cost functions to be comprised of a homogeneous function and a constant; in addition, the free flow travel times of all routes must be the same, although they can still be state-dependent. Under this condition, the average cost of all travelers $C(\q)$ can be written as an affine transformation of the weighted potential function $\potential(\q)$. From Theorem \ref{q_opt}, we know that any BWE $\qwe \in \Qwe(\lamb)$ minimizes the potential function $\potential(\q)$, and thus minimizes $C(\q)$ as well. Hence, $ \frac{\clamb}{\copt}=1$ for any size vector $\lamb$. This result also implies that $\clamb$ in \eqref{eq:average_cost_def} is a linear transformation of the value of the potential function in equilibrium, $\Plamb$. Recalling that $\Lambdag = \argmin_{\lamb} \Plamb$ from Lemma \ref{lemma_minimum_lambdag}, we can conclude that the routing game attains the minimum of the equilibrium average cost for any $\lamb \in \Lambdag$.

\begin{example}\label{eq_average_cost}
Fig. \ref{fig:soc_8_6_18_20_2} illustrates how $\clamb$ and $\copt$ vary with $\lamb$ for the routing game considered in Example \ref{benchmark_example}. In Fig. \ref{fig:soc_8_6_18_20_2}, The size vector $\lamb$ that minimizes $\clamb$ lies in regime $\Reone^{12}$. Fig. \ref{fig:soc_8_6_18_18_2} presents the same plot for the game in which $c_1^{n}(\l_1)=\l_1+20$, $c_1^{a}(\l_1)=3\l_1+20$; all other parameters remain unchanged. The sufficient condition in Proposition \ref{homo_bathtub} is satisfied in this case, so there is no inefficiency due to selfish routing.
    \end{example}


